Parameter Tuning for Self-optimizing Software at Scale

Efficiency of self-optimizing systems is heavily dependent on their optimization strategies, e.g., choosing exact or approximate solver. A choice of such a strategy, in turn, is influenced by numerous factors, such as re-optimization time, size of the problem, optimality constraints, etc. Exact solvers are domain-independent and can guarantee optimality but suffer from scaling, while approximate solvers offer a "good-enough" solution in exchange for a lack of generality and parameter-dependence. In this paper we discuss the trade-offs between exact and approximate optimizers for solving a quality-based software selection and hardware mapping problem from the scalability perspective. We show that even a simple heuristic can compete with thoroughly developed exact solvers under condition of an effective parameter tuning. Moreover, we discuss robustness of the obtained algorithm's configuration. Last but not least, we present a software product line for parameter tuning, which comprise the main features of this process and can serve as a platform for further research in the area of parameter tuning.

==> backup.tex <==
\section{Backup}
\begin{figure*}
	\centering
		\includegraphics[width=1.00\textwidth]{materials/RAHeuristicClassDiagram.pdf}
	\label{fig:RAHeuristicClassDiagram}
	\caption{Class diagram of the problem model}
\end{figure*}


The optimization problem to be solved by MQuAT is resource allocation. 
%\subsection{Problem Description (Dynamic)}

The main difference between a static and dynamic problems is an existence of changes in the problem model. Namely, it can be either addition/removal/change of request's requirements or addition/removal of a HW component/-s.

Although the re-generation of a new ILP w.r.t. aforementioned changes can be efficient~(see Sch\"{o}ne et.al.~\cite{schone2016incremental} for more details), the ILP should be solved completely. With the large problem models this computation can be very expensive. Therefore, an approach that can utilize the knowledge obtained during the previous iteration is preferable. 

%The problem model consists of the following components: 
%
%\textsl{\textbf{Incoming Requests}} with specified functional and non-functional properties~(NFP).
	%
%\textsl{\textbf{Software Components~(SWC)}} that provide required functionality, and have a set of implementations providing this functionality, but are different in their NFPs. Each implementation, in turn, can have different modes, i.e., configurations that influence its NFPs. SWC must require hardware components and may require other SWCs.
%
%\textsl{\textbf{Hardware Components~(HWC)}} comprise resources: CPU, memory, disk, network. They follow a life-cycle defining states and transitions between those states. States and transitions are annotated with respective power consumptions. A HWC may host multiple SWCs.
%
%The optimization problem presumes a construction of an optimal mapping of SWC to HWC w.r.t energy-efficiency for each timestamps. A timestamp, in this context, is expressed in a set of requests.

\subsection{Problem Description (Static)}

Each SWC implementation has a limited number of execution modes, which are defined exclusively for this implementation. 
For the sake of simplicity we substitute the hierarchical structure of implementations and respective modes by a flat structure: a single entity of implementation/mode combination. This combination helps to reduce the dimensionality of the search space (reduction of the number of decision variables) without a loss of granularity.

%Without a loss of problem model granularity we can substitute the implementation with and its possible modes by implementation/mode combinations and reduce the number of decision variables. % Needs a better explanation

The requests can be decomposed into computational tasks~$T.$ Each task $t \in T$ can be fulfilled by one of SWC implementations. 
Let $S$ be a set of SWC implementations with corresponding modes and $H$ the set of available hardware. 

A problem \textbf{solution} is a combination of two mappings: (1) an assignment of each task $t\in T$ to one (or more) SWC implementations $s\in S$; (2) a mapping of each $t$ to one hardware component (container) $h\in H$.

The SWC implementation assignment is denoted by the mapping $M_{SW}(t)=s$. The hardware allocation is denoted by $M_{HW}(t)=h$.

\textbf{Constraints} 

Let $R$ be a set of hardware resources~(CPU, memory, etc.) which is common to all of the HWCs in $H$. 
For a resource $r \in R$ we define $Cap(h, r)$ as an amount of the resource provided by $h$ and $Req_{resource}(t, s, r)$ as a required amount of the resource $r$ to run the SWC implementation $s$ for the task $t$.

Resource utilization for a single HWC:
\begin{equation}
U(h, r) = \sum_{t\in T,M_{HW}(t)=h,M_{SW}(t)=s} Req_{resource}(t, s, r)
\end{equation}

\textbf{C1.} Utilization constraint:
\begin{equation}
	U(h, r) \le Cap(h, r), \forall h \in H, r \in R
\end{equation}

According to the NFP nature, a QoS parameter can be specified as a minimum required or maximum allowed value. Let denote as $Req_{NFP}^{min|max}(t, p)$ the requested level of a nonfunctional property $p$ for a task $t$.
An SWC implementation~$s$ can provide NFP $p$ in the $Prov(s, p)$ amount. 

\textbf{C2.} User QoS satisfaction constraint (request NFP fulfillment):
\begin{equation}
\begin{aligned}
Req_{NFP}^{min}(t, p) \le Prov(s, p), &  \forall t \in T, p \in NFP, M_{SW}(t)=s  \\ % NFP needs to be changed to a character and defined in text.
Req_{NFP}^{max}(t, p) \ge Prov(s, p), & 
\end{aligned}
\end{equation}

\textbf{C3.} Subcomponent requirements satisfaction constraint:

\textbf{Objective Functions} 

\subsection{Particularities}

The described problem is not a classical bin packing. It is a two-level combinatorial optimization problem. The first level is selection of the software component hierarchy that can serve a respective request/-s. On the second level we search for an optimal hardware mapping to the selected software hierarchy. Despite this clear distinction we cannot treat hardware and software selections separately as they influence the score of the objective function only when bound together. 

Different nature of hardware and software components forbids treating them in the same way. The number HWC variables is restricted by the number of actual hardware resources, while we can create multiple instances of the same SWC.

The solution is a list of assignments of SWCs on HWCs. Each assignment contains one SWC and a respective HWC. The assignments can be represented as a tree that repeats the tree of dependencies between SWC requirements. 

Let us consider an example depicted in Figure~\ref{allocation_variants}. Here, we have a group of requests needed to be served. Request 1~(R1) can be fulfilled by an SWC of type A~(SWC-A). There exist N different implementations of SWC-A, each having up to M modes. Implementation 1 of SWC-A~(SWC-A-1) requires SWC-B, while SWC-A-N requires two SWCs: SWC-B and SWC-C. SWC-B, in turn requires SWC-D and SWC-E.

Now let us change an implementation of SWC-B. This change can induce significant changes to the SWC-hierarchy. In our example it creates an additional dependency to SWC-F from SWC-B, thus, altering a solution structure and consequently a search space structure. Note, that here we considered only the SWC-hierarchy. Addition of HWC mappings introduces even more complexity.

As the classical metaheuristics for combinatorial optimization can work only with a static search space structure, we need a special mechanism to mask these changes. For this, we calculate the maximum number of SWCs needed to serve each request, i.e., a worst-case scenario. Knowing this number we can create a list of empty assignments that can serve any scenario with the respective pool of requests. Then we randomly assign SWCs that can serve stated non-functional properties and HWCs that satisfy the respective SWCs; thus, obtaining a starting point for the local search(LS). 

%We construct an initial solution~(starting point for the MH) in the following way. First, we find the maximum size of the tree, needed to serve a request. Second, we create the list of empty assignments of the same size. Each assignment is marked as unnecessary to be filled, i.e., to contain an SWC and HWC. Third, we take random SWCs of the required type and fill the assignments one by one. If there are any empty assignments left, they do not influence the resulting score of the solution. Finally, we complete the assignments with random HWCs. 

Each iteration of any LS is based on two main notions: \emph{move} and \emph{score calculation}. Move is a change of a planning variable that provides a new solution, i.e., explores the search space. Score calculation is necessary to assess the quality of the obtained solution and, thus, helps to decide which move to take. 

There are two types of moves in our MH: HWC- and SWC-move. Former is just a random substitution of an assigned HWC by a different one, while latter is a bit more complicated. After changing a random SWC at a random level of hierarchy it presumes a modification of requirements for the dependent SWCs, removal of the obsolete assignments and addition of the new ones. Note, that the addition of new assignments means not a new assignments of SWC-HWC pairs creation, but unblocking the existent assignments, thus, allowing to utilize them at the current stage of the LS.

After the move is performed, the score calculation takes place. We iterate through all the component assignments and check whether the underlying SWCs and HWCs are complying with the stated requirements. We utilize a so-called hardsoft score\footnote{\url{https://docs.optaplanner.org/7.0.0.Final/optaplanner-docs/html_single/index.html\#hardSoftScore}} in our MH. It allows to split the objective function~(energy consumption) and other requirements while comparing two solutions. If any constraint, such as missing or unsatisfying qualities of an SWC or HWC, is violated, the hard score is decreasing. The soft score summarizes the energy consumption of all HWCs executing picked SWCs. Better score means a bigger number of both hard and soft scores. As the optimization problem we try to solve is a minimization problem, the score is represented by negative values. Negative hard score means that some hard constraints are violated and zero, when no constraint is broken. The soft score in our example never reaches zero as the HWCs cannot serve SWCs without consuming any energy. Therefore, the optimal soft score is a minimum energy consumption with the negative sign. The optimal score looks as follows: 
\begin{equation}
0 \, \texttt{hard} \, / \, -min(energy\_consumption) \, \texttt{soft}.
\end{equation}

Note, that the score $0 \,  \texttt{hard} \, / \, -10 \, \texttt{soft}$ is better than \\ $-1 \,  \texttt{hard} \, / \, -1000 \, \texttt{soft}$ as the hard score has a higher priority than soft. By using such a scoring strategy we can ensure the knowledge whether the obtained solution is valid~(serves all the requests).   



\begin{figure}%
\includegraphics[width=\columnwidth]{materials/AllocationVariants}%
\caption{Different variants of SWC hierarchies based on a selected implementation}%
\label{allocation_variants}%
\end{figure}


